Envy-freeness in 3D Hedonic Games

We study the problem of partitioning a set of agents into coalitions based on the agents' additively separable preferences, which can also be viewed as a hedonic game. We apply three successively weaker solution concepts, namely envy-freeness, weakly justified envy-freeness, and justified envy-freeness. In a model in which coalitions may have any size, trivial solutions exist for these concepts, which provides a strong motivation for placing restrictions on coalition size. In this paper, we require feasible coalitions to have size three. We study the existence of partitions that are envy-free, weakly justified envy-free, and justified envy-free, and the computational complexity of finding such partitions, if they exist. We present a comprehensive complexity classification, in terms of the restrictions placed on the agents' preferences. From this, we identify a general trend that for the three successively weaker solution concepts, existence and polynomial-time solvability hold under successively weaker restrictions.

==> old.tex <==
% \documentclass[preprint,12pt]{elsarticle}

% \journal{}

% \usepackage{amsmath}
% \usepackage{amssymb}

% \let\proof\relax
% \let\endproof\relax
% \usepackage{amsthm}

% % suppress some unfixable warnings
% \usepackage{silence}
% \WarningFilter{hyphenat}{***}
% \WarningFilter{thmtools}{LLNCS support}

% \usepackage{hyperref}
% \usepackage[noend]{algpseudocode}
% \usepackage{algorithm}

% \usepackage{soul}
% \usepackage{complexity}
% \usepackage{graphicx}
% \usepackage{enumitem}
% \usepackage{tikz}
% \usepackage[htt]{hyphenat}
% \usepackage[most]{tcolorbox}
% \usepackage{ltablex}
% \usepackage{multirow}
% \usepackage{lipsum}
% \usepackage{changepage}
% \usepackage{tabularx}
% \usepackage{mathrsfs}
% \usepackage{readarray}

% % adjust the margins for MATCH-UP
% % \usepackage{geometry}
% % \geometry{
% %   a4paper,         % or letterpaper
% %   textwidth=12.2cm,  % llncs has 12.2cm
% %   textheight=19.3cm, % llncs has 19.3cm
% %   heightrounded,   % integer number of lines
% %   hratio=1:1,      % horizontally centered
% %   vratio=2:3,      % not vertically centered
% % }

% \hyphenation{preferences}

% \usepackage{thmtools}
% \usepackage{thm-restate}

% \usepackage{xcolor,colortbl,bm,graphicx,adjustbox}
% \usepackage{afterpage}

% \declaretheorem[name=Theorem]{thm}
% \declaretheorem[name=Definition, style=remark]{definition}
% \declaretheorem[name=Lemma]{lem}
% \declaretheorem[name=Proposition]{prop}
% \declaretheorem[name=Observation]{observation}
% \declaretheorem[style=remark, numbered=no, name=Proof sketch, qed=$\square$]{proofsketch}
% \declaretheorem[style=remark, numbered=no, name=Remark]{myremark}

% \declaretheoremstyle[
% notebraces={}{},
% headpunct={},
% headformat={\NAME\ \NUMBER.~\NOTE},
% headfont=\bfseries, 
% postheadhook = {\hspace*{0pt}},
% % postheadspace = \newline, 
% spaceabove = 0.5cm, 
% spacebelow = 0.5cm]{myproblemstyle}
% \declaretheorem[style=myproblemstyle, name=Problem]{myproblem}

% \declaretheoremstyle[
% notebraces={}{},
% headpunct={},
% headformat={\NAME\ \NUMBER.~\NOTE},
% headfont=\itshape, 
% postheadhook = {\hspace*{0pt}},
% % postheadspace = \newline, 
% spaceabove = 0.5cm, 
% spacebelow = 0.5cm]{mydefinitionstyle}
% \declaretheorem[style=mydefinitionstyle, name=Definition]{mydefinition}

% \newcommand{\inp}{\textit{Input: }} 
% \newcommand{\outp}{\textit{Output: }}
% \newcommand{\ques}{\textit{Question: }}

% \newcommand{\algorithmfont}[1]{\textsf{#1}}
% \newcommand{\myoplus}{\oplus}

% % https://tex.stackexchange.com/q/440184
% \usepackage{eqparbox}
% \newcommand{\matheqbox}[2]{\eqmakebox[#1][c]{$\displaystyle#2$}}

% \algdef{S}[WHILE]{WhileNoDo}[1]{\algorithmicwhile\ #1}%	
% \algrenewcommand\algorithmicindent{1.0em}

% % made this to allow for indented multiline assignments in algorithms
% % based on various stackoverflow answers
% \usepackage{silence}
% \WarningFilter{etex}{Extended allocation}
% \usepackage{linegoal}
% \makeatletter
% \algnewcommand{\myhackyalgorithmbox}[1]{ \parbox[t]{\linegoal}{#1}
% }
% \makeatother

% % breakable algorithm
% % https://tex.stackexchange.com/a/33869
% \makeatletter
% \newenvironment{breakablealgorithm}
%   {% \begin{breakablealgorithm}
%    \begin{center}
%      \refstepcounter{algorithm}% New algorithm
%      \hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
%      \renewcommand{\caption}[2][\relax]{% Make a new \caption
%        {\raggedright\textbf{\fname@algorithm~\thealgorithm} ##2\par}%
%        \ifx\relax##1\relax % #1 is \relax
%          \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
%        \else % #1 is not \relax
%          \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
%        \fi
%        \kern2pt\hrule\kern2pt
%      }
%   }{% \end{breakablealgorithm}
%      \kern2pt\hrule\relax% \@fs@post for \@fs@ruled
%    \end{center}
%   }
% \makeatother


% % line comments in pseudocode
% \makeatletter
% \algnewcommand{\LineComment}[1]{\State \(\triangleright\) \myhackyalgorithmbox{#1}
% }
% \makeatother

% % checkmarks
% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\maynotexist}{\ding{55}}%

% % prevent leading indentation in entire algorithmic
% \usepackage{xpatch}
% \makeatletter
% \xpatchcmd{\algorithmic}
%   {\ALG@tlm\z@}{\leftmargin\z@\ALG@tlm\z@}
%   {}{}
% \makeatother

% \usetikzlibrary{arrows,decorations.markings,decorations.pathreplacing,patterns,matrix,calc,positioning,backgrounds,arrows.meta,shapes,decorations.markings,fadings,bending,decorations.pathmorphing}

% % this is to fix an issue with tikz angles
% % see https://tex.stackexchange.com/a/260833
% \makeatletter
% \tikzset{
%   reset label anchor/.code={%
%     \let\tikz@auto@anchor=\pgfutil@empty
%     \def\tikz@anchor{#1}
%   },
%   reset label anchor/.default=center,
%   every label/.append style={reset label anchor}
% }
% \makeatother

% \tikzset{darrow/.style={decoration={
%   markings,
%   mark=at position .2 with {\arrowreversed{angle 90[width=2.5mm]}},
%   mark=at position .8 with {\arrow{angle 90[width=2.5mm]}},
%   }
%   ,postaction={decorate}}}

% \tikzset{darrow12/.style={decoration={
%   markings,
%   mark=at position {0.2*\pgfdecoratedpathlength} with {\arrowreversed{angle 90[width=2.5mm]}},
%   mark=at position {0.8*\pgfdecoratedpathlength-0.4mm} with {\arrow{angle 90[width=2.5mm]}},
%   mark=at position {0.8*\pgfdecoratedpathlength+0.4mm} with {\arrow{angle 90[width=2.5mm]}},
%   }
%   ,postaction={decorate}}}
  
% \tikzset{darrow22/.style={decoration={
%   markings,
%   mark=at position {0.2*\pgfdecoratedpathlength-0.4mm} with {\arrowreversed{angle 90[width=2.5mm]}},
%   mark=at position {0.2*\pgfdecoratedpathlength+0.4mm} with {\arrowreversed{angle 90[width=2.5mm]}},
%   mark=at position {0.8*\pgfdecoratedpathlength-0.4mm} with {\arrow{angle 90[width=2.5mm]}},
%   mark=at position {0.8*\pgfdecoratedpathlength+0.4mm} with {\arrow{angle 90[width=2.5mm]}},
% %   mark=between positions 0.8 and 1.0 step 3mm with {\arrow{angle 90[width=2.5mm]}},
%   }
%   ,postaction={decorate}}}

% \tikzset{-->-/.style={decoration={
%   markings,
%   mark=at position .8 with {\arrow{angle 90[width=2.5mm]}}},postaction={decorate}}}
  
% \tikzset{-<--/.style={decoration={
%   markings,
%   mark=at position .8 with {\arrow{angle 90[width=2.5mm]}}},postaction={decorate}}}
  
% \tikzset{->-/.style={decoration={
%   markings,
%   mark=at position .5 with {\arrow{angle 90[width=2.5mm]}} },postaction={decorate}}}

% \tikzset{--->/.style={decoration={
%   markings,
%   mark=at position 1 with {\arrow{angle 90[width=2.5mm]}} },postaction={decorate}}}

% \tikzset{
%   nat/.style     = {fill=white,draw=none,ellipse,minimum size=0.3cm,inner sep=1pt},
% }

% % made this myself
% \usepackage[most]{tcolorbox}
% \newcommand{\paranote}[2] {
% \begin{tcolorbox}[enhanced, parbox=false, colback=#1, drop shadow]
%     \begin{minipage}{\textwidth}
%         {\sffamily Note: #2}
%     \end{minipage}
% \end{tcolorbox}
% \medskip
% }

% % do not need todonotes for submission
% \iffalse
%     \usepackage[textsize=small,textwidth=4cm,shadow]{todonotes}
%     \newcommand{\accom}[1]{\todo[color=orange!75!white]{\'{A}: #1}} 
%     \newcommand{\mmcom}[1]{\todo[inline, color=green!25!white]{M: #1}}
%     \newcommand{\agnes}[1]{\textcolor{orange}{#1}}
%     \usepackage[normalem]{ulem}%Agnes: This package allows us to strike out text
% \fi

% % Agnes: Here we can control the paragraph settings.
% % \makeatletter
% % \renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
% %                                     {0.6ex \@plus1ex \@minus.2ex}%
% %                                     {-1em}%
% %                                   {\normalfont\normalsize\bfseries}} %{\normalfont\normalsize\itshape}}
% % \makeatother

% % uncomment to show margin guides
% % \usepackage{showframe}
% % \renewcommand*\ShowFrameLinethickness{0.5pt}
% % \renewcommand*\ShowFrameColor{~\color{black!10}}

% % Used for displaying a sample figure. If possible, figure files should
% % be included in EPS format.
% %
% \renewcommand\UrlFont{\color{blue}\rmfamily}

% \pgfdeclarelayer{background}
% \pgfdeclarelayer{foreground}
% \pgfsetlayers{background,main,foreground}

% \makeatletter
% \pgfkeys{%
%   /tikz/on layer/.code={
%     \def\tikz@path@do@at@end{\endpgfonlayer\endgroup\tikz@path@do@at@end}%
%     \pgfonlayer{#1}\begingroup%
%   }%
% }
% \makeatother

% \tikzset{edge from parent/.append style={\solutionconceptsdiagramarrow}}

% \newcommand{\arrowwithtext}[1] {%
%     \begin{pgfonlayer}{foreground}
%     \draw[line width=0.3mm] (0.0,0.0) -- (-0.125cm, 0.15cm);
%     \draw[line width=0.3mm] (0.0, 0.0) -- (-0.125cm, -0.15cm);
%     \node[draw,circle,white,fill,minimum size=0.45cm] (background) at (-0.5, 0.0) {};
%     \node (anonymousnode) at (background) {#1};
%     \end{pgfonlayer}
% }  

% \newcommand\solutionconceptsdiagramarrow{-Straight Barb[length=1.4mm]}

% \newcommand{\myvaluationarrow}{%
%     \draw (0.0,0.0) -- (-0.125cm, 0.15cm);
%     \draw (0.0, 0.0) -- (-0.125cm, -0.15cm);
% }

% \newcommand{\myvaluationarrowreversed}{%
% \begin{scope}[xscale=-1.0]
% \myvaluationarrow
% \end{scope}
% }

% \tikzset{darrow/.style={decoration={
%   markings,
%   mark=at position .2 with {\myvaluationarrowreversed},
%   mark=at position .8 with {\myvaluationarrow},
%   }
%   ,postaction={decorate}}}
  
% % convex hull stuff (used for dashedcontainerthing) https://tex.stackexchange.com/questions/70999/highlight-a-group-of-nodes-in-a-tikz-tree/71000#71000
% \newcommand{\convexpath}[2]{
% [   
%     create hullnodes/.code={
%         \global\edef\namelist{#1}
%         \foreach [count=\counter] \nodename in \namelist {
%             \global\edef\numberofnodes{\counter}
%             \node at (\nodename) [draw=none,name=hullnode\counter] {};
%         }
%         \node at (hullnode\numberofnodes) [name=hullnode0,draw=none] {};
%         \pgfmathtruncatemacro\lastnumber{\numberofnodes+1}
%         \node at (hullnode1) [name=hullnode\lastnumber,draw=none] {};
%     },
%     create hullnodes
% ]
% ($(hullnode1)!#2!-90:(hullnode0)$)
% \foreach [
%     evaluate=\currentnode as \previousnode using \currentnode-1,
%     evaluate=\currentnode as \nextnode using \currentnode+1
%     ] \currentnode in {1,...,\numberofnodes} {
%   let
%     \p1 = ($(hullnode\currentnode)!#2!-90:(hullnode\previousnode)$),
%     \p2 = ($(hullnode\currentnode)!#2!90:(hullnode\nextnode)$),
%     \p3 = ($(\p1) - (hullnode\currentnode)$),
%     \n1 = {atan2(\y3,\x3)},
%     \p4 = ($(\p2) - (hullnode\currentnode)$),
%     \n2 = {atan2(\y4,\x4)},
%     \n{delta} = {-Mod(\n1-\n2,360)}
%   in 
%     {-- (\p1) arc[start angle=\n1, delta angle=\n{delta}, radius=#2] -- (\p2)}
% }
% -- cycle
% }
% \newcommand\dashedcontainerthing[1]{%
% \readlist*\nodes{#1}%
% \begin{scope}[on background layer]
%     \ifthenelse{\nodeslen>1}{
%         \draw[thick, densely dashed] \convexpath{#1}{0.353cm};
%         \fill[white] \convexpath{#1}{9.6pt};
%     }{
%         \node[draw, thick, circle, densely dashed, minimum size=20pt] (anonymousnode) at (\nodes[1]) {};
%     }
% \end{scope}
% }

% \definecolor{enclosure_color}{rgb}{0.6,0.6.,0.6}
% \definecolor{figurecolourschemewt1_adjusted}{rgb}{0.8,0.8,0.8}
% \definecolor{figurecolourschemewt1}{rgb}{0.5,0.5,0.5}
% \definecolor{figurecolourschemewt2}{rgb}{0.5,0.0,0.5}
% \definecolor{figurecolourschemewt3}{rgb}{0,0,0}
% \definecolor{figurecolourschemewt4}{rgb}{0,0,1}
% \definecolor{figurecolourschemewt5}{rgb}{0,1,0}
% \definecolor{figurecolourschemewt6}{rgb}{1,0,0}

% \newcommand{\figurecolorschemewtonename}{grey}
% \newcommand{\figurecolorschemewttwoname}{purple}
% \newcommand{\figurecolorschemewtthreename}{black}
% \newcommand{\figurecolorschemewtfourname}{blue}
% \newcommand{\figurecolorschemewtfivename}{green}
% \newcommand{\figurecolorschemewtsixname}{red}

% \def\porschenxsatvariant/{$\text{X3SAT}_{+}^{\,=3}$}
% \def\iwjnomaxdegreetwofamily/{$\mathcal{I}^\star$}

% \usepackage[normalem]{ulem} % this allows us to strike out text

% \title{Envy-freeness in 3D Hedonic Games\texorpdfstring{\footnote{This work was supported by the Engineering and Physical Sciences Research Council (Doctoral Training Award 2125850), OTKA grant K128611, and the J\'anos Bolyai Research Fellowship.}}{}}


% \author[inst1]{\'Agnes Cseh}
% \address[inst1]{Institute of Economics, Centre for Economic and Regional Studies, Budapest, 1097, Hungary}

% \author[inst2]{Michael McKay}
% \author[inst2]{David Manlove}

% \address[inst2]{School of Computing Science, University of Glasgow, Glasgow, G12 8QQ, United~Kingdom}
            
% \begin{document}
% % \input{writing_conventions}
% % \pagebreak
% \begin{frontmatter}

% %

% %
% %\titlerunning{Abbreviated paper title}
% % If the paper title is too long for the running head, you can set
% % an abbreviated paper title here
% %
% % \author[agnes]{\inst{1}\orcidID{0000-0003-4991-2599} \and
% % Michael McKay\inst{2}\orcidID{0000-0003-1496-7434} \and
% % David Manlove\inst{2}\orcidID{0000-0001-6754-7308}}
% % %
% % \authorrunning{Cseh et al.}
% % % First names are abbreviated in the running head.
% % % If there are more than two authors, 'et al.' is used.
% % %
% % \affiliation[agnes]{Centre for Economic and Regional Studies, Institute of Economics, Hungary\\
% % \email{cseh.agnes@krtk.hu} \and
% % School of Computing Science, University of Glasgow, UK\\ \email{m.mckay.1@research.gla.ac.uk}, \email{david.manlove@glasgow.ac.uk}}

            
% %
% % \maketitle              % typeset the header of the contribution
% %
% \begin{abstract}
% \input{sections/abstract}
% \end{abstract}
% \begin{keyword}
% Coalition formation \sep Hedonic games \sep Multidimensional roommates \sep Envy-freeness.
% \end{keyword}
% \end{frontmatter}

% \input{sections/intro}
% \input{sections/preliminaries}
% \input{sections/theoretical_results/theoretical_results}
% \input{sections/conclusion}
% \input{sections/acknowledgements}

% \bibliographystyle{elsarticle-num}
% \bibliography{mybib}

% \end{document}


==> style/sn-article-template/sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


